Divergent Search for Few-Shot Image Classification

When data is unlabelled and the target task is not known a priori, divergent search offers a strategy for learning a wide range of skills. Having such a repertoire allows a system to adapt to new, unforeseen tasks. Unlabelled image data is plentiful, but it is not always known which features will be required for downstream tasks. We propose a method for divergent search in the few-shot image classification setting and evaluate with Omniglot and Mini-ImageNet. This high-dimensional behavior space includes all possible ways of partitioning the data. To manage divergent search in this space, we rely on a meta-learning framework to integrate useful features from diverse tasks into a single model. The final layer of this model is used as an index into the `archive' of all past behaviors. We search for regions in the behavior space that the current archive cannot reach. As expected, divergent search is outperformed by models with a strong bias toward the evaluation tasks. But it is able to match and sometimes exceed the performance of models that have a weak bias toward the target task or none at all. This demonstrates that divergent search is a viable approach, even in high-dimensional behavior spaces.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = sample-sigconf.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


sample-sigconf.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.thm *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> notes.tex <==
\begin{table}[]
\begin{tabular}{lllll}
\hline
Algorithm (way-shot) (5,5) & test & train & & \\ \hline
ACAI CACTUs-MAML               & 87.78 &       &  &  \\ 
BiGAN CACTUs-MAML              & 78.66 &       &  &  \\ \hline

%MCC 1k                         & 75.0  & 78.02 &  &  \\
%MCC 1k 5 testshots               & 75.91  & 78.92 &  &  \\
%MCC 100k 5 testshots             & 61.85  & 63.45 &  &  \\

%6E-1
%MCC 1k 10 testshots               & 76.70  & 78.98 &  &  \\

%5E-1
%MCC 1k 10 testshots               & 78.41  & 80.79 &  &  \\

%5E-1 - preventing single-class batches
%MCC 1k 10 testshots               & 77.58  & 80.13 &  &  \\

%5E-1 - preventing single-class batches, extra dense step
%MCC 1k 10 testshots               & 75.32  & 77.45 &  &  \\

%7.5E-1 - preventing single-class batches
%MCC 1k 10 testshots               & 70.72  & 73.15 &  &  \\

%5E-1 - preventing single-class batches, dense reset
%MCC 1k 10 testshots               & 56.02  & 61.60 &  &  \\

%5E-1 
%MCC 1k 10 testshots               & 76.15 & 78.86 &  &  \\

%5E-1, 9E-1 - entropy min/max
%MCC 1k 10 testshots               & 67.63 & 70.43 &  &  \\
%2.5E-1, 7.5E-1 - entropy min/max
%MCC 1k 10 testshots               & 66.69 & 69.59 &  &  \\

%4E-1, 8E-1 - scale vars
%MCC 1k 10 testshots               & 77.06 & 79.69 &  &  \\

%4E-1, 8E-1 - scale vars clip
%MCC 1k 10 testshots               & 74.57 & 77.81 &  &  \\

%4E-1, 6E-1, 8E-1 - coteach 5E-1
%MCC 1k 10 testshots               & 63.10 & 66.52 &  &  \\

%MCC 100k                       & 59.22 & 61.73 &  &  \\
%MCC 100k 5 shots               & 58.27 & 60.53 &  &  \\
%MCC 100k 5 shots               & 58.27 & 60.53 &  &  \\ \hline
%MMCC trans 1k 10 testshots               & 81.47  & 84.15 &  &  \\ \hline
%MMCC trans 1k 10 testshots no reset aux  & 81.82  & 84.72 &  &  \\

%skill search
Proposed                        & 81.15  & 83.53 &  &  \\ \hline

%supervised-reptile 1k & 91.04 & 92.10 &  &  \\
supervised-reptile trans 1k & 93.53 & 94.45 &  &  \\ \hline
%random init & 59.13 & 61.38 &  &  \\ 
random init trans & 64.29 & 66.28 &  &  \\ \hline
%Why is cactus-maml paper's from scratch accuracy so much higher? It essentially beats nearly all of their pretrained methods
\end{tabular}
\end{table}




\begin{figure*}[htb]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/rfs100k_m55_19c.pdf}
		\caption{\textit{Fully Supervised}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
	    \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rUMTRA6k_m55_19c.pdf}
		\caption{\textit{Low-Aug UMTRA}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rNC6k_m55_19cA.pdf}
		\caption{\textit{Proposed}}
	\end{subfigure}
	%\hspace*{\fill}
	
	%new row
	\begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/rfs100k_m55_26c.pdf}
		\caption{\textit{Fully Supervised}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
	    \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rUMTRA6k_m55_26c.pdf}
		\caption{\textit{Low-Aug UMTRA}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rNC6k_m55_26cA.pdf}
		\caption{\textit{Proposed}}
	\end{subfigure}
	%\hspace*{\fill}
	
	%new row
	\begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/rfs100k_m55_2c.pdf}
		\caption{\textit{Fully Supervised}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
	    \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rUMTRA6k_m55_2c.pdf}
		\caption{\textit{Low-Aug UMTRA}}
	\end{subfigure}
	%\hspace*{\fill}
	\begin{subfigure}[t]{0.32\linewidth}
		\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{figures/rNC6k_m55_2cAredo.pdf}
		\caption{\textit{Proposed}}
	\end{subfigure}
	%\hspace*{\fill}
	
	\caption{{Example t-SNE plots using the logit outputs for 10 test images per class after fine-tuning on $N=5, K=5$ examples. Each row is a different task. Green/red borders indicate whether images were correctly/incorrectly classified. The fully supervised approach is able to group images by class characteristics that are invariant to transformations. The proposed divergent approach appears to rely on more generic features such as spatial frequency, pose, or image style. Best viewed digitally.}}
	\label{figures:tsne}		
\end{figure*}







%instead of just novelty, qd introduces an objective of quality. qd is used extensively in reinforcement learning problems but there you have an agent with somewhat limited behaviors and a state space which has highly semantic information. e.g. moving to a state with a distance displacement, this new state implies some kind of movement which causes the agent to travel. 
%some similarities to open ended evolution bc it searches for new problems and tries to solve them, which inturn leads to more complex problems. also bc it is qd without any human specified quality metric.


%There are several strategies for learning features without labels, of which self-supervision and clustering are among the most popular. Self-supervised tasks attempt to reconstruct, generate, or re-assemble images, which helps with learning the features contained within a given image. This bypasses the need for any information on the relationship \textit{between} images. Alternatively, clustering attempts to discover these relationships by grouping similar images (typically based on a distance metric). Unfortunately, the features learned by self-supervision may not be useful for discriminating between images; meanwhile clustering may form groups based on features that are not of interest (e.g. lighting conditions or background structure). Szerlip et al. proposed another option, a search for features that discriminate between images in as many ways as possible \ref{szerlip}. This does not mean separating images into progressively finer categories; it instead aims to find features that divide the data in new ways. For example, the same set of hand written characters could be organized by size, shape, or style, each time producing different partitions. Many representation learning methods (e.g. infoGAN \ref{Chen2016}) also aim to learn these dimensions of variation, but Szerlip et al. are unique in their approach which is explicitly divergent. In theory, a divergent search could discover more subtle features because it continually seeks novel partitions rather than converging to the cardinal dimensions of variation. Such features are often necessary for more difficult tasks, for example spotting a disease which only appears in a small region of the image. These types of features are notoriously difficult to discover unsupervisedly %without supervision
%where image differences, such as pose, dominate the learned features. So far, this unsupervised divergent search has only been demonstrated in very restricted settings (i.e. using single-layer networks and requiring a pass of the entire training dataset to characterize feature novelty - for further details see related works). The goal of this work is to perform unsupervised divergent search within more modern frameworks and to provide solutions to the problems associated with scaling up. 
%Recent work in meta-learning has aimed to learn a set of features that is generally useful (or quickly adaptable) for a range of tasks which may have never been presented during training \ref{finn,nichol}. Typically this is used in a supervised setting, but this framework has attractive properties for unsupervised learning. Specifically, it grants us the freedom to train on a range of \textit{mock} tasks (derived without human-labelling) and still learn useful features for a (human-labelled) target task, even if the mock tasks never matched the target task. This insight has already been exploited by Hsu et al. who use self-supervised and clustering based methods to \textit{propose} mock tasks \ref{hsu}. In their extensive experiments they find that the performance of the meta learner is directly related to the performance of the self-supervised/clustering method, i.e. the quality of the proposed mock tasks \ref{hsu}. Training a separate unsupervised proposal network helps to bootstrap performance at the cost of being cumbersome and time consuming. In this work, we implement a divergent search strategy within this meta learning framework. This eliminates the need for separate training stages and continually evolves to learn new partitions.

%Scaling divergent search to state-of-the-art meta learning frameworks presents several challenges. Most divergent search strategies have been developed with reinforcement learning problems in mind, for example controlling a walking robot. In such cases, it is relatively simple to define a space of meaningful behaviors spanning movement in different directions, at different speeds, or even with differing gaits. In image classification, there is not an obvious equivalent. Szerlip et al. opted for measuring a feature detector's response to the entire training dataset and searched for feature detectors that divided the training data in novel ways. While this may work for a 1-layer feature detector \ref{Szerlip}, modern neural networks are powerful enough to divide data precisely in arbitrary ways \ref{zhang}. As such, the behavior space is vast and mostly meaningless. For example, a set of only 100 images can be partitioned into 5 non-empty sets in roughly \num{6.6e67} different ways; many of these divisions may be useful for different tasks but \textit{most} of these are likely useless. 

%noise for exploration is effective in reinforcement learning because the search space is relatively small and the reward signal is very meaningful
%Many divergent search strategies rely on i) behavioral descriptors, to measure the relative novelty of solutions, and ii) niche archives, to collect diverse solutions. However, it is not obvious how to measure behavioral novelty in an image classification task. Szerlip et al. opted for measuring a (single layer) feature detector's response to every image in the training set (forming a 1xN vector, where N is the number of training images). Scaling up to larger datasets and deeper networks quickly becomes impractical. Also, deep networks can learn random labels perfectly \ref{Zhang}; this means that there are network weights that can partition the data in  arbitrary ways that do not correspond to any useful 
%with more complex images and more complex features, this method may learn to 

%we frame unsupervised learning as a continual search for novel, high-quality behavior.

%we don't have a strong, meaningful, reward signal like in reinforcement learning, e.g. speed, distance travelled, etc.  

%advantage over sota and demonstrating it

%clustering based on finetuning to non-normal
%or infogan comparison
%pretraining teacher on self-supervised task? 
%gecco, fasp miccai, clustering

%This is difficult to scale to deeper networks and larger datasets.  
%scaling to deeper networks gives more discriminative power, but also flexibility that comes with that means there are way too many diverse features
%also there are too many diverse behaviors which can eventually become meaningless
%having a larger network also makes it more difficult to form a niche archive. there is also likely a large overlap. We draw on meta learning approach mentioned above to accumulate all features into a single network, making finetuning straightforward. 
%rather than trying to exploit the distribution to push the benchmark performance, here we attempt to study the impact of the distribution on NC. This helps to indicate which types of data distributions may be most suitable
%character displacement


%To gain more varied mock tasks, they perform k-means clustering several times on top of the self-supervised/clustering embeddings, each time randomly scaling the dimensions of the embedding space \ref{hsu}. However, their results indicate that the difference between running k-means once and 100 times is small and that the primary determinant of performance of the meta learner is the performance of the self-supervised/clustering method, i.e. the quality of the proposed mock tasks \ref{hsu}. 
 
%different unsupervised methods work better for different datasets, leading to a lengthy process of trial and error (involving training both the proposal network and meta learner).

%While it is attractive to generalize to unseen tasks (including unseen classes), this is not explicitly our goal, because in the unsupervised setting there are no human-specified tasks presented during training. Instead, the quality of interest is that these meta learning frameworks can learn features from a range of tasks that are helpful for a new unseen task. This affords us the freedom of training on many different tasks which may not match the desired test task, yet still learning something useful.  
%unique because explicitly divergent 
%self teaching
%different because it tries to always find more complex tasks
%instead of illuminating across dimensions that are predetermined or iteratively learned, this approach tries to escape the space covered by all previous solutions
%
%weakness - num of steps
%weakness - since not separate niches, noisy solutions will impact the quality of the end resulting model

%many evolutionary studies assume the environment is a static factor, similarly labels are often considered fixed. But more complex studies consider the environment as malleable, susceptible to change by the organisms. However, since we are only interested in diverse high quality behaviors, where behavior is defined as different groupings of the images. 

%search for novel, high quality behavior 

%Successful organisms not only adapt to their environment, but also shape their surroundings. This in turn affects selection pressures. This feedback loop produces niches where organisms perform advanced functions and thrive in their (tailored) environment. For example, a squirrel may modify its environment by accumulating and storing food (reducing the instability of resource availability). As a result, features useful for hiding food, such as claws for digging, might become more advantageous.
%As an open-ended evolutionary process, it is difficult to control which niches emerge; but the quality and diversity of resulting behaviors can form a repertoire that is broadly useful for many different tasks. The purpose of this work is to investigate whether this type of feedback system can produce a repertoire that is useful in image classification. 

%Consider the Omniglot dataset, a large range of hand written characters from different languages. These images can be grouped in many ways, e.g. character size, components such as loops or lines, or writing style. However, it is often difficult to get a single set of labels for data, let alone an exhaustive set of all sensible groupings. Also the exact target task e.g. character recognition, style/language classification, author/forgery detection, may not be known in advance; or we may want a single system that is broadly prepared for any of these tasks.
%conversely, if we train an unsupervised system and it does not give a useful representation, the entire system must be retrained and it is not obvious how to adjust hyperparameters to extract the features we are interested in.
%Here we investigate whether `niche construction' can learn discriminative features for all types of groupings, without using any labels. 

%The motivation behind the proposed method is aligned with the field of quality diversity (QD). However, existing QD methods require users to specify the dimensions of behavior or rely on sensor signals (e.g. in robotics) to automatically characterize behaviors. In image classification, it is not obvious how to characterize `behaviors' or how to relate behaviors relative to each other. The latter is a key requirement for divergent search which aims to explore the solution space beyond the area that has already been illuminated. Szerlip et al. proposed a divergent search for image classification \ref{Szerlip}, using a feature's response to the entire training dataset to characterize its behavior. Unfortunately this may be difficult to scale to larger networks and larger datasets. 



%the organism, the competitor, and the resource. The resource network aims to find a novel and generalizable partition behavior by the end of an inner loop iteration. As with most QD algorithms, the loss function (for the resource) includes a novelty component and a quality component. The novelty objective is typically driven by a comparison to an archive of accumulated solutions; in this case, the competitor network acts as the archive. It is only able to modify the parameters in its last layer, $\theta_\textrm{fc}$, essentially re-purposing existing features to best match the resource's partition behavior.

%\begin{equation}
%\mathcal{L}_{\textrm{competitor}} = KL(R(x;w)||C(x'_u;w)).
%\min_{\theta_\textrm{fc}}\; JS(R(x;\phi)||C(x;\theta))
%\label{equation:competitor_loss}
%\end{equation}

%The competitor network tries to minimize the Jensen-Shannon (JS) divergence shown in Eqn. \ref{equation:competitor_loss}, where $R$ and $C$ are resource and competitor networks respectively, with parameters $\phi$ and $\theta$ respectively, and identical input images $x$. Meanwhile, the resource network tries to maximize this JS divergence. It must find partitions that the existing features, $\theta$, are not equipped to replicate. 
%more broadly useful features defend a larger niche - though this does not strictly protect them from replacement..

%Using novelty search on its own could lead to accumulation of mostly low-utility features. There are countless arbitrary ways to group a set of images, e.g. based on noise, that will satisfy novelty, but will not lead to learning broadly useful features. Unfortunately it is difficult to derive a gradient for the quality of a behavior without any human-specified reference behavior. Even if two networks are trained to make consistent predictions (with one another), this does not necessarily constrain behavior at all. However, if this learned behavior is still consistent for images that were not involved in training, then their features may exhibit more robust behavior. As such, consistency can act as a surrogate measure for quality, but it cannot directly provide a gradient. Evolutionary computation excels in this regard. Fitness functions without gradients can still be sampled and a population-based gradient can be estimated. In this sense, our approach is akin to an evolutionary strategy; but each instead of random mutations,
%To make the behaviors more likely to generalize, we can regularize the resource and organism network with the same prior. 
%Instead, we can try to  the resource network needs some form of regularization. In QD algorithms there is often an overarching objective/fitness function used to measure the quality of a solution. For example, if designing virtual locomotive `creatures', novelty could be explored across dimensions of height, mass, and number of joints, while fitness could reward the distance the creature was able to travel\ref{lehman}. In our case, fitness and novelty are not measured on orthogonal axes, instead partition behavior agreement is used for both. This is the role of the organism network, to draw the resource network toward more generalizable behaviors. 

%\begin{equation}
%\mathcal{L}_{\textrm{competitor}} = KL(R(x;w)||C(x'_u;w)).
%\min_{\psi}\; JS(R(x;\phi)||O(x;\psi))
%\label{equation:organism_loss}
%\end{equation}

%As with the competitor, the organism tries to minimize the JS divergence shown in Eqn. \ref{equation:organism_loss}, but the organism is free to change all of its parameters ($\psi$). Note that at the start of every inner loop iteration, $\psi = \theta = \theta^i$, in other words the competitor and organism start at the same initialization point ($\theta^i$). The resource network ($\phi$) starts at a random mutation of the same initialization point, $\phi = \theta^i + s\eta$. Safe mutations\cite{lehman2018safe} are used to scale ($s$) the parameter space noise ($\eta$) into a reasonable range for each parameter. 
%add details of how to use organism network, backprop through gradient steps?

%\begin{equation}
%\mathcal{L}_{\textrm{competitor}} = KL(R(x;w)||C(x'_u;w)).
%\min_{\phi}\; -JS(R(x;\phi)||C(x;\theta)) + JS(R(x;\phi)||O(x;\psi))
%\min_{\phi}\; -JS(R||C) + JS(R||O)
%\label{equation:resource_loss}
%\end{equation}

%The resource network is optimized according to a combination of the two objectives (Eqn. \ref{equation:resource_loss}). Each network is updated iteratively up to a set number of steps, \textit{num\_interactions}. This gives final parameter values, $\theta^f$, $\phi^f$, and $\psi^f$, for the competitor, resource, and organism respectively. At the end of this process, the organism network is reset to the initialization point ($\psi = \theta^i$) and then re-trained on its own following Eqn. \ref{equation:organism_loss} for a very limited number of steps, \textit{inner\_reptile\_steps}. This results in the parameter setting $\tilde{\psi}$. This reset step must be done because the final position of the organism network, $\tilde{\psi}$, must be near the initialization point, $\theta^i$, for the inter-task aggregation (outer loop) to work effectively. This also mimics the standard algorithm of Reptile\cite{nichol2018first}, but using the resource network outputs in place of ground truth labels. By using the same setup we keep all other factors constant,
%can isolate the labels as the primary difference, 
%allowing us to more directly compare i) the quality of the resource network outputs to ii) the quality of the ground truth labels. 



%the organism network is reset to the initialization point ($\psi = \theta^i$) and then re-trained on its own following Eqn. \ref{equation:organism_loss} for a very limited number of steps, \textit{inner\_reptile\_steps}. This results in the parameter setting $\tilde{\psi}$. This reset step must be done because the final position of the organism network, $\tilde{\psi}$, must be near the initialization point, $\theta^i$, for the inter-task aggregation (outer loop) to work effectively. This also mimics the standard algorithm of Reptile\cite{nichol2018first}, but using the resource network outputs in place of ground truth labels. By using the same setup we keep all other factors constant,
%can isolate the labels as the primary difference, 
%allowing us to more directly compare i) the quality of the resource network outputs to ii) the quality of the ground truth labels. 


%The standard outer loop for Reptile simply takes the final parameter values of the (organism) network, $\tilde{\psi}$, from each inner loop iteration and calculates the mean, $\overline{\psi} = \frac{1}{n}\sum_{i=1}^{n} \tilde{\psi}_i$. Using ground truth labels it is natural to weight each task equally, but in an unsupervised setting some tasks may be higher quality than others. As such a weighted mean is used, as shown in Eqn. \ref{equation:psi_mean}.


%Measuring the value of a task (i.e. the teacher behavior) is done by comparing  how well the archive and learner models were able to match the teacher behavior. Since the archive is restricted to only using its fully connected layer, $\theta_{fc}$, the learner model is handicapped with dropout~\cite{srivastava2014dropout} in its final layer to make for a fairer comparison.%While the archive is restricted to only using its fully connected layer, $\theta_{fc}$, the learner is able to freely change all of its parameters. Without any regularization, the learner can fit any arbitrary behavior, making this comparison meaningless. As such, dropout~\cite{srivastava2014dropout} is used in the fully connected layer of the learner. 


%There are several factors which may explain this. First, given the model's limited capacity, it is not able to accumulate a complete archive of encountered behaviors. This violates an assumption used in the theoretical analysis of novelty search by Doncieux et al., namely that an unbounded archive is available~\cite{doncieux2019novelty}. Even so, pre-training on random behaviors is 
%Second, according to their analysis, as the behavior space grows relative to the specificity of the goal behaviors, the probability that the


%Having a divergent task based on a history of previously explored behaviors could help reduce oscillation around certain behaviors and ensure that new ones are can help avoid oscillations in this high-dimensional behavior space. %prevent oscillations, imperfect optimization 

